Efficient Continual Pre-training for Building Domain Specific Large Language Models

Large language models (LLMs) have demonstrated remarkable open-domain capabilities. LLMs tailored for a domain are typically trained entirely on domain corpus to excel at handling domain-specific tasks. In this work, we explore an alternative strategy of continual pre-training as a means to develop domain-specific LLMs over an existing open-domain LLM. We introduce FinPythia-6.9B, developed through domain-adaptive continual pre-training on the financial domain. Continual pre-trained FinPythia showcases consistent improvements on financial tasks over the original foundational model. We further explore simple but effective data selection strategies for continual pre-training. Our data selection strategies outperform vanilla continual pre-training's performance with just 10% of corpus size and cost, without any degradation on open-domain standard tasks. Our work proposes an alternative solution to building domain-specific LLMs cost-effectively.

==> tables/finqa.tex <==
\begin{table*}[h]
\centering
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
                                            & \textbf{Tokens}       & FinQA     \\
                                            &                       & Acc        \\
\midrule
\textbf{Pythia 1B}                          & 0                     & 0.00314 (0.00284) \\
\midrule
\textbf{DACP}                               & 2.39B (10\%)          & \\
\textbf{DACP}                               & 23.9B (100\%)         & 0.00017 (0.00035)\\
\midrule
\textbf{TACP}                               & 0.24M                 & 0.00022 (0.00038)  \\
\midrule
\multicolumn{3}{c}{\textbf{Hard Sampling}}\\
\midrule
\textbf{ETS-DACP}                           & 2.39B (10\%)          & 0.00454 (0.0023) \\
\textbf{ETA-DACP-ppl}                       & 2.39B (10\%)          & \\
\textbf{ETA-DACP-ent}                       & 2.39B (10\%)          & \\
\textbf{ETS-DACP-com}                       & 2.39B (10\%)          & 0.00087 (0.00110) \\
\midrule
\multicolumn{3}{c}{\textbf{Soft Sampling}}\\
\midrule
\textbf{ETS-DACP}                           & 2.39B (10\%)          & 0.00070 (0.00085)\\
\textbf{ETA-DACP-ppl}                       & 2.39B (10\%)          &  \\
\textbf{ETA-DACP-ent}                       & 2.39B (10\%)          & \\
\textbf{ETS-DACP-com}                       & 2.29B (10\%)          & 0.00366 (0.00294) \\
\bottomrule
\end{tabular}
}
\caption{Performance on FinQA. Accuracy mean and standard deviation are computed over 5 runs. }
\label{tab:finqa}
\end{table*}
